cube2net: Efficient Query-Specific Network Construction with Data Cube Organization

Networks are widely used to model objects with interactions and have enabled various downstream applications. However, in the real world, network mining is often done on particular query sets of objects, which does not require the construction and computation of networks including all objects in the datasets. In this work, for the first time, we propose to address the problem of query-specific network construction, to break the efficiency bottlenecks of existing network mining algorithms and facilitate various downstream tasks. To deal with real-world massive networks with complex attributes, we propose to leverage the well-developed data cube technology to organize network objects w.r.t. their essential attributes. An efficient reinforcement learning algorithm is then developed to automatically explore the data cube structures and construct the optimal query-specific networks. With extensive experiments of two classic network mining tasks on different real-world large datasets, we show that our proposed cube2net pipeline is general, and much more effective and efficient in query-specific network construction, compared with other methods without the leverage of data cube or reinforcement learning.

==> sec-app.tex <==
%!TEX root = cube2net.tex
\section*{Appendices}
%This proof is based on the assumption that the pre-trained word embedding $\mathcal{U}_W$ has captured word semantics in the vocabulary $\mathcal{W}$, so that $\forall w_i, w_j \in \mathcal{W}, ||\mathbf{u}_{w_i}-\mathbf{u}_{w_j}||^2_2<\epsilon S(w_i, w_j)$, where $S(w_i, w_j)$ is the semantic gap between $w_i$ and $w_j$. 
%
%Based on $S(w_i, w_j)$, we further define the semantic gaps among labels. 
%Specifically, $\forall l_i, l_j \in \mathcal{L}^p$, where $p\in\mathcal{P}$ is any cube dimension, suppose $l_i = \{w_i^1, w_i^2, \ldots, w_i^{K_i}\}$, where $K_i$ is the number of words in $l_i$; $l_j = \{w_j^1, w_j^2, \ldots, w_j^{K_j}\}$, where $K_j$ is the number of words in $l_j$, the semantic gap $S(l_i, l_j)$ can then be defined as
%\begin{align}
%S(l_i, l_j) = \sum_{k_i=1}^{K_i}\sum_{k_j=1}^{K_j} S(w_i^{k_i}, w_j^{k_j}).
%\end{align} 
%
%Now we first prove that the label embedding $\mathcal{U}_L$ captures the label semantics, so that $\forall l_i, l_j \in \mathcal{L}^p, ||\mathbf{u}_{l_i} - \mathbf{u}_{l_j}||_2^2 \leq \epsilon S(l_i, l_j)$. It holds when $K_i=K_j$, which means $l_i$ and $l_j$ have the same number of words. Although in practice this condition is not always satisfied, since most labels have similar numbers of words, we find the algorithm still works well.
%
%\begin{proof}
%For the label embeddings $\mathcal{U}_L$, ($\forall \mathbf{u}_l \in \mathcal{U}_L, \mathbf{u}_l=\sum_{k=1}^{K} \mathbf{u}_{w_l^k}$), we have
%\begin{align}
%&||\mathbf{u}_{l_i}-\mathbf{u}_{l_j}||^2_2 \nonumber\\
%= & ||\sum_{k_i=1}^{K_i}\mathbf{u}_{w_i^{k_i}} - \sum_{k_j=1}^{K_j}\mathbf{u}_{w_j^{k_j}}||^2_2\nonumber\\
%= & \sum_{k_i=1}^{K_i} \mathbf{u}_{w_i^{k_i}}^T \mathbf{u}_{w_i^{k_i}} + \sum_{k_j=1}^{K_j}\mathbf{u}_{w_j^{k_j}}^T\mathbf{u}_{w_j^{k_j}} \nonumber\\
%& + 2 \sum_{k_i^1 \neq k_i^2; k_i^1, k_i^2=1}^{K_i} \mathbf{u}_{w_i^{k_i^1}}^T \mathbf{u}_{w_i^{k_i^2}} +
%2 \sum_{k_j^1 \neq k_j^2; k_j^1, k_j^2=1}^{K_j} \mathbf{u}_{w_j^{k_j^1}}^T \mathbf{u}_{w_j^{k_j^2}} \nonumber\\
%& - 2 \sum_{k_i=1}^{K_i} \sum_{k_j=1}^{K_j} \mathbf{u}_{w_i^{k_i^1}}^T \mathbf{u}_{w_j^{k_j^1}},\\
%\nonumber\\
%&\text{and}\nonumber\\
%\nonumber\\
%&\sum_{k_i=1}^{K_i} \sum_{k_j=1}^{K_j} || \mathbf{u}_{w_i^{k_i}} - \mathbf{u}_{w_j^{k_j}} ||^2_2 \nonumber\\
%= & K_j \sum_{k_i=1}^{K_i} \mathbf{u}_{w_i^{k_i}}^T  \mathbf{u}_{w_i^{k_i}} + K_i \sum_{k_j=1}^{K_j} \mathbf{u}_{w_j^{k_j}}^T  \mathbf{u}_{w_j^{k_j}} \nonumber\\
%& - 2 \sum_{k_i=1}^{K_i} \sum_{k_j=1}^{K_j} \mathbf{u}_{w_i^{k_i}}^T \mathbf{u}_{w_j^{k_j}}.
%\end{align}
%
%Subtracting the two terms, we have\\
%\begin{align}
%&\sum_{k_i=1}^{K_i} \sum_{k_j=1}^{K_j} || \mathbf{u}_{w_i^{k_i}} - \mathbf{u}_{w_j^{k_j}} ||^2_2 - ||\mathbf{u}_{l_i}-\mathbf{u}_{l_j}||^2_2 \nonumber\\
%= & (K_j - 1) \sum_{k_i=1}^{K_i} \mathbf{u}_{w_i^{k_i}}^T  \mathbf{u}_{w_i^{k_i}} + (K_i - 1) \sum_{k_j=1}^{K_j} \mathbf{u}_{w_j^{k_j}}^T  \mathbf{u}_{w_j^{k_j}} \nonumber\\
%&- 2 \sum_{k_i^1 \neq k_i^2; k_i^1, k_i^2=1}^{K_i} \mathbf{u}_{w_i^{k_i^1}}^T \mathbf{u}_{w_i^{k_i^2}} - 2 \sum_{k_j^1 \neq k_j^2; k_j^1, k_j^2=1}^{K_j} \mathbf{u}_{w_j^{k_j^1}}^T \mathbf{u}_{w_j^{k_j^2}} \nonumber\\
%= & (K_j - K_i)(\sum_{k_i=1}^{K_i} \mathbf{u}_{w_i^{k_i}}^T  \mathbf{u}_{w_i^{k_i}} - \sum_{k_j=1}^{K_j} \mathbf{u}_{w_j^{k_j}}^T  \mathbf{u}_{w_j^{k_j}}) \nonumber\\
%& + \sum_{k_i^1 \neq k_i^2; k_i^1, k_i^2=1}^{K_i} || \mathbf{u}_{w_i^{k_i^1}} - \mathbf{u}_{w_i^{k_i^2}} ||^2_2 \nonumber\\
%& + \sum_{k_j^1 \neq k_j^2; k_j^1, k_j^2=1}^{K_j} || \mathbf{u}_{w_j^{k_j^1}} - \mathbf{u}_{w_j^{k_j^2}} ||^2_2 \nonumber\\
%\geq & 0.\\\nonumber
%\end{align}
%
%Therefore, we have\\
%\begin{align}
%&||\mathbf{u}_{l_i}-\mathbf{u}_{l_j}||^2_2 \leq \sum_{k_i=1}^{K_i} \sum_{k_j=1}^{K_j} || \mathbf{u}_{w_i^{k_i^1}} - \mathbf{u}_{w_j^{k_j^1}} ||^2_2 \nonumber\\
%\leq & \epsilon \sum_{k_i=1}^{K_i}\sum_{k_j=1}^{K_j} S(w_i^{k_i}, w_j^{k_j}) = \epsilon S(l_i, l_j) \qedhere. 
%\end{align}
%\end{proof}
%
%Moreover, $\forall c_i, c_j \in \mathcal{C}$, suppose $c_i = \{l_i^1, l_i^2, \ldots, l_i^{P}\}$, and $c_j = \{l_j^1, l_j^2, \ldots, l_j^{P}\}$, where $P$ is the number of cube dimensions, we then define the semantic gap $S(c_i, c_j)$ as
%\begin{align}
%S(c_i, c_j) = \sum_{p=1}^{P} S(l_i^p, l_j^p).
%\end{align} 
%
%Now we prove that the cell embedding $\mathcal{U}_C$ captures the cell semantics, so that $\forall c_i, c_j \in C, ||\mathbf{u}_{c_i} - \mathbf{u}_{c_j}||_2^2 \leq \epsilon S(c_i, c_j)$.
%
%\begin{proof}
%For the cell embeddings $\mathcal{U}_C$, ($\forall \mathbf{u}_{c} \in \mathcal{U}_C, \mathbf{u}_{c}=[\mathbf{u}_{l_{c}^1}, \ldots, \mathbf{u}_{l_{c}^P}]$, where $[\ldots]$ denotes vector concatenation), the proof is trivial because the norm of a concatenated vector equals to the sum of the norms of its components, \ie,
%\begin{align}
%& ||\mathbf{u}_{c_i} - \mathbf{u}_{c_j}||^2_2 \nonumber\\
%= & \sum_{p=1}^P ||\mathbf{u}_{l_i^{p}} - \mathbf{u}_{l_j^{p}}||^2_2 \nonumber\\
%\leq & \epsilon \sum_{p=1}^P S(l_i^p, l_j^p) = \epsilon S(c_i, c_j)\qedhere.
%\end{align}
%\end{proof}
%\newpage

%Continue with our toy example on DBLP in Figure \ref{fig:cube}, where the gradually changing colors represent the changing cell semantics. 
%According to Theorem \ref{th:cube}, our novel cell embedding process maps the discrete data cube cells into a continuous embedding space, where cells with similar semantics lie close. 
%Together with the examples and theoretical analysis in Section \ref{sec:rl}, we show that such a property further guarantees the efficient and effective exploration of cube structures and construction of query-specific networks without the need of exhaustive search over all cube cells.

%\begin{figure*}
%\centering
%\subfigure[Precision]{
%\includegraphics[width=0.245\textwidth]{figures/prec_nvout.png}}
%\hspace{-8pt}
%\subfigure[Recall]{
%\includegraphics[width=0.245\textwidth]{figures/rec_nvout.png}}
%\hspace{-8pt}
%\subfigure[Runtime / log(s)]{
%\includegraphics[width=0.245\textwidth]{figures/time_nvout.png}}
%\hspace{-8pt}
%\subfigure[Network Size / log(\#)]{
%\includegraphics[width=0.245\textwidth]{figures/size_nvout.png}}
%\caption{\textbf{Performance of network construction for link prediction on the NVOUT Yelp subset.}}
%\label{fig:nvout}
%\end{figure*}






